GREENER: A Tool for Improving Energy Efficiency of Register Files

Graphics Processing Units (GPUs) maintain a large register file to increase the thread level parallelism (TLP). To increase the TLP further, recent GPUs have increased the number of on-chip registers in every generation. However, with the increase in the register file size, the leakage power increases. Also, with the technology advances, the leakage power component has increased and has become an important consideration for the manufacturing process. The leakage power of a register file can be reduced by turning infrequently used registers into low power (drowsy or off) state after accessing them. A major challenge in doing so is the lack of runtime register access information. This paper proposes GREENER (GPU REgister file ENErgy Reducer): a system to minimize leakage energy of the register file of GPUs. GREENER employs a compile-time analysis to estimate the run-time register access information. The result of the analysis is used to determine the power state of the registers (ON, SLEEP, or OFF) after each instruction. We propose a power optimized assembly instruction set that allows GREENER to encode the power state of the registers in the executable itself. The modified assembly, along with a run-time optimization to update the power state of a register during execution, results in significant power reduction. We implemented GREENER in GPGPU-Sim simulator, and used GPUWattch framework to measure the register file's leakage power. Evaluation of GREENER on 21 kernels from CUDASDK, GPGPU-SIM, Parboil, and Rodinia benchmarks suites shows an average reduction of register leakage energy by 69.04% and maximum reduction of 87.95% with a negligible number of simulation cycles overhead (0.53% on average).

==> Makefile <==
TGT=OptimizeRegPower

BIBTEX=bibtex
LATEX=pslatex
DVIPS=dvips
PS2PDF=ps2pdf
# Ignore these for now!
PS2PDF_OPTS=-dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress 
LATEX_OPTS=-interaction=nonstopmode -halt-on-error
LATEX_OPTS=

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"


.PHONY: all clean

all: $(TGT).pdf

$(TGT).dvi : $(TGT).tex Sections/*.tex OptimizeRegPower.bib runtime.c
	$(LATEX) $(LATEX_OPTS) $(TGT).tex
	@if(grep "There were undefined references" $(TGT).log > /dev/null);\
	then \
		$(BIBTEX) $(TGT).aux; \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex; \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex; \
	fi
	@if(grep "Rerun" $(TGT).log > /dev/null);\
	then \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex;\
	fi

$(TGT).ps: $(TGT).dvi
	$(DVIPS) -j0 $<

$(TGT).pdf: $(TGT).ps
	$(PS2PDF) $<

clean:
	$(RM) $(TGT).aux $(TGT).log   \
		$(TGT).blg $(TGT).bbl \
		$(TGT).dvi $(TGT).out \
		$(TGT).pdf $(TGT).ps


==> Sections/00-todo.tex <==
\tbd{
\section*{TODO before final submission}
\begin{enumerate}
\item replace {\em access range} by {\em live range}
\item check space after \Release.
\item Spell check
\item remove this section
\item replace resource with scratchpad accordingly
\item Write hardware requirement section, and compute the number of extra bits require to model the latency of \Release\ instruction
\end{enumerate}
}


==> Sections/06-Analysis.tex <==
\section{Time Complexity} \label{sec:analysis}
\tobedone{
Add about time compliexity of Compiler Analysis
}

